One loop integration with hypergeometric series by using recursion relations

General one-loop integrals with arbitrary mass and kinematical parameters in $d$-dimensional space-time are studied. By using Bernstein theorem, a recursion relation is obtained which connects $(n+1)$-point to $n$-point functions. In solving this recursion relation, we have shown that one-loop integrals are expressed by a newly defined hypergeometric function, which is a special case of Aomoto-Gelfand hypergeometric functions. We have also obtained coefficients of power series expansion around 4-dimensional space-time for two-, three- and four-point functions. The numerical results are compared with LoopTools for the case of two- and three-point functions as examples.

==> macrol.tex <==
%%-------------------------------------------------
\newcommand{\textem}[1]{{\em#1}}
\newenvironment{Theorem}[2]{\par\textbf{Theorem #1} #2 ~ }{%
    $\square$\par}
\newenvironment{Corollary}[2]{\par\textbf{Corollary #1} #2 ~ }{%
    $\square$\par}
\newenvironment{Lemma}[2]{\par\textbf{Lemma #1} #2 ~ }{%
    $\square$\par}
\newenvironment{Definition}[2]{\par\textbf{Definition #1} \textbf{#2} ~ }{%
    $\square$\par}
\newenvironment{Remark}[2]{\par\textbf{Remark #1} #2 ~ }{%
    $\square$\par}
\newenvironment{Annotation}[2]{\par\textbf{(Ãí)#1} #2 ~ }{%
    $\square$\par}
\newenvironment{Item}{\par\noindent $\bullet$ ~ }{%
    $\square$\par}
\newenvironment{Example}[2]{\par\textbf{Example #1} #2 ~ }{%
    $\square$\par}
\renewcommand{\Re}{\mathrm{Re}}
% \DeclareMathOperator*{\Re}{Re}
\renewcommand{\Im}{\mathrm{Im}}
% \DeclareMathOperator*{\Im}{Im}
\newcommand{\Ref}[1]{#1}
\newcommand{\RefEq}[1]{(#1)}
\newenvironment{Itemize}{%
  \begin{list}{}{%
    \setlength{\topsep}{0pt}%
    \setlength{\parsep}{0pt}%
    \setlength{\itemsep}{0pt}%
  }}{\end{list}}
\DeclareMathOperator*{\Card}{card}
\DeclareMathOperator*{\Id}{id}
\newcommand{\Hyp}{\operatorname{Hyp}}
\newcommand{\Vol}{\operatorname{Vol}}

\newcommand{\PAR}{\par\vspace{2em}}
% \newcommand{\ITEM}{\par\noindent{\(\blacksquare\)}~}
% \newcommand{\ITEM}{{\setlength{\parskip}{2em}\par\noindent{\(\blacksquare\)}~}}
\newcommand{\GS}{\SetComplex_{\text{gen}}^A}
% \newcommand{\IE}{i \varepsilon}
\newcommand{\DirSimplex}[1]{\langle#1\rangle}
%---------------------------------------------------------------
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bc}{\begin{center}}
\newcommand{\ec}{\end{center}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
\newcommand{\benu}{\begin{enumerate}}
\newcommand{\eenu}{\end{enumerate}}
\newcommand{\bdes}{\begin{description}}
\newcommand{\edes}{\end{description}}
\newcommand{\nn}{\nonumber}

%---------------------------------------------------------------


==> macros.tex <==
\newtheorem{theorem}{定理}[section]
\newtheorem{lemma}{補題}[section]
\newcommand{\Proof}{\noindent\par\textbf{証明}\quad}
\newcommand{\EndProof}{(\textbf{証明終わり})}

\newcommand{\VOne}{\mathbb{I}}
\newcommand{\Den}{{\cal D}}
\newcommand{\EDen}{{\cal E}}
\newcommand{\NDen}{{\cal E}}
\newcommand{\EIR}{{\epsilon_{IR}}}
\newcommand{\EUV}{{\epsilon}}
\newcommand{\IE}{{i \varepsilon}}
\DeclareMathOperator{\Log}{\operatorname{Log}}
\newcommand{\Set}[1]{\{#1\}}
\newcommand{\SetIn}[2]{\left\{#1 \,\left|\; #2 \right.\right\}}
\newcommand{\SetInL}[2]{\left\{\left.#1 \,\right| \, #2 \right\}}
\newcommand{\SetNatural}{\mathbb{N}}
\newcommand{\SetInteger}{\mathbb{Z}}
\newcommand{\SetRational}{\mathbb{Q}}
\newcommand{\SetReal}{\mathbb{R}}
\newcommand{\SetComplex}{\mathbb{C}}
\newcommand{\SetProjective}{\mathbb{P}}
\newcommand{\CConjg}[1]{\overline{#1}}
% \newcommand{\SetInteger}{\mathbf{Z}}
% \newcommand{\SetReal}{\mathbf{R}}
% \newcommand{\SetComplex}{\mathbf{C}}
\newcommand{\Binom}[2]{\left(\hspace{-0.3em}\begin{array}{c}
                       #1\\#2\end{array}\hspace{-0.3em}\right)}
\newcommand{\Ideal}[1]{\langle#1\rangle}
\newcommand{\Inc}[2]{\left(#1\right)_{#2}}
\newcommand{\Dec}[2]{\left[#1\right]_{#2}}
\newcommand{\Li}{\operatorname{Li}}
\newcommand{\HP}{\operatorname{H}}
\DeclareMathOperator{\Tr}{\operatorname{Tr}}
% \DeclareMathOperator{\Det}[1]{\operatorname{det}(#1)}
\newcommand{\Det}[1]{\left|#1\right|}
\newcommand{\TP}[1]{{#1}^{\text{T}}}
\newcommand{\IBeta}[3]{B(#1,#2;#3)}
\newcommand{\IBetaBar}[3]{\bar{B}(#1,#2;#3)}
\newcommand{\Arc}{\operatorname{Arc}}
\newcommand{\Arg}{\operatorname{Arg}}
\DeclareMathOperator{\Partial}{\overline{\partial}}
\newcommand{\Eq}{\;=\;}

% Hypergeometric functions
\newcommand{\FG}[4]{F\left(#1,#2;#3;#4\right)}      % Gauss
\newcommand{\FA}[4]{F_1\left(#1,#2;#3;#4\right)}    % Appell's F_1
\newcommand{\FD}[4]{F_D\left(#1,#2;#3;#4\right)}    % Laurichella's F_D

\newcommand{\OpUp}[1]{{\cal T}^{+}_{#1}}
\newcommand{\OpDown}[1]{{\cal T}^{-}_{#1}}
\newcommand{\OpDiff}{{\cal D}}

\DeclareMathOperator{\Mat}{\operatorname{Mat}}
\DeclareMathOperator{\Sign}{\operatorname{Sign}}
\DeclareMathOperator{\sign}{\operatorname{sign}}

\DeclareMathOperator{\Mod}{\operatorname{Mod}}
\DeclareMathOperator{\Ker}{\operatorname{Ker}}
\DeclareMathOperator{\Image}{\operatorname{Im}}
\DeclareMathOperator{\Hom}{\operatorname{Hom}}
\DeclareMathOperator{\Dim}{\operatorname{dim}}
\DeclareMathOperator{\Aut}{\operatorname{Aut}}
\DeclareMathOperator{\GCD}{\operatorname{GCD}}
\DeclareMathOperator*{\Supp}{\operatorname{supp}}
\DeclareMathOperator{\Resultant}{\operatorname{Res}}
\DeclareMathOperator{\ConvexHull}{\operatorname{CH}}
\DeclareMathOperator{\Kern}{\operatorname{Kern}}
\DeclareMathOperator{\Ann}{\operatorname{Ann}}
\DeclareMathOperator{\ord}{\operatorname{ord}}
\newcommand{\Ord}[1]{{\cal O}(#1)}
\newcommand{\Rooti}[2]{{\cal R}_{#1}(#2)}
\newcommand{\Root}[1]{{\cal R}(#1)}

\newcommand{\Norm}[1]{\|#1\|}

\newcommand{\Frac}[2]{\displaystyle\frac{\displaystyle{#1}}{\displaystyle{#2}}}
\newcommand{\Comment}[1]{}
% \newcommand{\Comment}[1]{(#1)}

\newcommand{\Def}[1]{\textbf{#1}\index{#1}}
\newcommand{\SymDef}[2]{#1\index{#2}}

% \newcommand{\ITEM}{\par\noindent{\(\blacksquare\)}~}
\newcommand{\ITEM}{{\setlength{\parskip}{2em}\par\noindent{\(\blacksquare\)}~}}

